Studying Ad Library Integration Strategies of Top Free-to-Download Apps

In-app advertisements have become a major revenue source for app developers in the mobile app ecosystem. Ad libraries play an integral part in this ecosystem as app developers integrate these libraries into their apps to display ads. In this paper, we study ad library integration practices by analyzing 35,459 updates of 1,837 top free-to-download apps of the Google Play Store. We observe that ad libraries (e.g., Google AdMob) are not always used for serving ads -- 22.5% of the apps that integrate Google AdMob do not display ads. They instead depend on Google AdMob for analytical purposes. Among the apps that display ads, we observe that 57.9% of them integrate multiple ad libraries. We observe that such integration of multiple ad libraries occurs commonly in apps with a large number of downloads and ones in app categories with a high proportion of ad-displaying apps. We manually analyze a sample of apps and derive a set of rules to automatically identify four common strategies for integrating multiple ad libraries. Our analysis of the apps across the identified strategies shows that app developers prefer to manage their own integrations instead of using off-the-shelf features of ad libraries for integrating multiple ad libraries. Our findings are valuable for ad library developers who wish to learn first hand about the challenges of integrating ad libraries.

==> Background.tex <==
Ad networks often provide documentation or tutorial in their websites that demonstrate the integration process of ad libraries for displaying advertisement into apps.

To integrate ad libraries, app developers need to perform the four steps as follows:
\textbf{Step 1: Create an account in an ad network and register apps.} At first, app developers create an account in an ad network and register their apps.     
The ad network generates an unique app id for each registered apps. 
   
\textbf{Step 2: Add permissions and activities of an ad library in the app's AndroidManifest.xml.} 
To download ad contents (e.g., prefetching images or video advertisements) and to display contextual advertisements (e.g., user's location based advertisements), ad libraries require permission.
App developers add the required permissions for ad libraries in the \textit{AndroidManifest.xml} file using \textit{$<$uses-permission$>$} elements. 

\textbf{Step 3: Define the activity.}
To display advertisements in a separate screen (e.g., full screen advertisements or video advertisements), ad libraries have their own activites. 
App developers need to add the activities of ad libraries in the \textit{AndroidManifest.xml} file.

\textbf{Step 4: Integrate ad libraries with the app code.} This step has 4 practices as follows: (1) single ad library integration strategy, (2) mediation integration strategy, (3) non-mediation integration strategy and (4) mixed integration strategy.
App developers use the single ad library integration strategy to integrate a single ad library with the app code. 
To integrate multiple ad libraries, app developers use any of the integration strategy among the other three strategies.
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/Background_ad_integration_strategy.pdf}
    \caption{Mediation and non-mediation integration strategy}
    \label{fig:ad_integration_strategy}
\end{figure*}

\begin{enumerate}

    \item\textbf{Single ad library integration strategy.} In this integration strategy, app developers add a single ad library of an ad network into their apps.
    App developers directly call the required APIs of the ad library in the activities of the apps (i.e., app code) to initialize the ad library and to show advertisements.
    
    \item \textbf{Mediation integration strategy.}
    In this integration strategy, app developers add multiple ad libraries of different ad networks into their apps.
    Figure~\ref{fig:ad_integration_strategy}(a) shows the mediation integration strategy.
    As shown in the Figure~\ref{fig:ad_integration_strategy}(a),
    app developers include an ad library of the ad network that supports mediation platform.
    The mediation platform of the ad library enables app developers to integrate only the ad library with their apps that automatically communicates with other ad networks to display advertisements from them.
    The main advantage of using mediation integration strategy is that app developers do not require to write codes manually to integrate each added ad library from different ad networks with their apps.
    Rather, app developers only integrate the ad library that provides mediation platform with their apps to display advertisement from different ad networks.
    So, mediation integration strategy ease the maintenance process of multiple ad libraries.
    However, mediation integration strategy has some drawbacks such as mediation platform  (1) does not support all ad networks (for example, the mediation platform of the Google AdMob can not display advertisements from the Amazon Mobile Ads), 
    (2) slows the ad fetching and the ad display process, and
    (3) does not provide the feature to control ad frequency. 

    \item \textbf{Non-mediation integration strategy.}
    In this integration strategy, app developers integrate more than one ad library with their apps.
    To integrate multiple ad libraries with their app code, app developers do not use the mediation platform of the ad library. 
    Rather, they implement their own codes to communicate multiple ad libraries to display advertisements.
    Figure~\ref{fig:ad_integration_strategy}(b) shows the non-mediation integration strategy. 
    As shown in the Figure~\ref{fig:ad_integration_strategy}, the app code directly communicate to the integrated ad libraries to display advertisements.
    In this integration strategy, app developers have two options to communicate with multiple ad libraries: (1) writing codes for each ad library to show ads in different app screens (i.e., activities) and (2) writing codes to prioritize the ad libraries based on some criteria (e.g., user's location) and select the appropriate ad library to show ads in the app screens.
    So, app developers require more maintenance effort to manage multiple ad libraries in the non-mediation integration.
    However, non-mediation integration strategy help app developers control ad frequency in the apps. 
    \item \textbf{Mixed integration strategy.}
    In this integration strategy, app developers combine both the mediation integration strategy and the non-mediation strategy to integrate multiple ad libraries with their apps. 
    The mixed integration strategy creates a balance of integrating multiple ad libraries.
    For example, app developers can ease the maintenance process of multiple ad libraries by using the mediation integration strategy.
    They also get benefited by the non-mediation integration strategy as they can manually integrate the profitable ad libraries and control the ad frequency.
     
    
    
\end{enumerate}


==> RQ3.tex <==
\noindent\emph{Motivation:}
In Section~\ref{sec:RQ2_Results}, we observe that app developers need to do a lot of work to integrate more than one ad library.
In this section, we study the evolution of ad library usage. In particular, we study the ad library migration and rollback and study the updates where app developers change ad-call-site code and update ad libraries.
Understanding about how ad library usage evolve over time can help ad library developers to gain knowledge about the dynamic nature of ad market and the maintenance effort of ad libraries.

\noindent\emph{Approach:}
In this section, at first, we describe the process for identifying ad library migration and rollback cases. Then, we detail our approach for identifying updates where app developers update ad-related code (e.g., ad-call-site code and ad libraries).
Finally, we describe the process for identifying emergency updates where app developers update ad-related code.

\textbf{Identify ad library migration and rollback cases.}
To identify ad library migration and rollback cases of an ad-displaying app, we compared the integrated ad libraries of the app's update $U_{i}$ and it's subsequent update $U_{i+1}$.
We identify an ad library migration case if the following rules are satisfied:
\begin{enumerate}
    \item There is a difference in the integrated ad libraries of the update $U_{i}$ and $U_{i+1}$
    \item An ad library \textit{$L_{1}$} is removed  in the update $U_{i}$ and a new ad library \textit{$L_{2}$} is added in the update $U_{i+1}$.
\end{enumerate}
We identify an ad library rollback case if the  following rules are satisfied:
\begin{enumerate}
    \item There is a difference in the integrated ad libraries of the update $U_{i}$ and $U_{i+1}$
    \item An ad library \textit{$L_{1}$} is added in the update  $U_{i+1}$ 
    \item The added ad library \textit{$L_{1}$} was integrated in the previous updates of $U_{i-1}$
\end{enumerate}
At the end of this step, we identified all the ad library migration and rollback cases for each of the studied apps.

\textbf{Identify app updates where app developers update ad-call-site code and ad libraries.}
To study how app developers maintain ad libraries, we consider the app updates where app developers update ad libraries and the code for integrating these ad libraries (i.e., ad-call-site code).
To identify the app updates where app developer update ad libraries and ad-call-site code, we followed a similar approach to the one presented by Ruiz et al.~\cite{updates_ad_library}:

For each update of an app that serve ads, we analyzed the byte code of the generated Jars from the APKs of the update using the BCEL tool~\cite{BCEL}.
We generated class signatures for each of the classes and compared them to identify the changes between two classes.
We followed a similar approach of software bertilonage to generate the class signatures and to compare them~\cite{bertillonage}.
In particular, we followed three steps to identify the update of ad libraries and ad-call-site code.

\noindent\textbf{Step 1: Generate class signatures for ad library code.}
At first, we identified ad library classes if they exist under the package of the ad library.
Then, for each identified ad library in an update of an app, we generated signatures for all classes of the ad library.
To generate a signature of a class, we constructed a string by combining the fully qualified class name (e.g., combination of package name and class name), method names of the class and parameter types of the methods. 
At the end of this step, we generated class signatures of all the classes of the integrated ad libraries.

\noindent\textbf{Step 2: Generate class signatures for ad-call-site code.}
We define ad-call-site code as the statements of app code that call ad library methods.
To locate ad-call-site code, we used the BCEL tool to identify all statements from the classes of app code that call ad library methods.
Then, for each class of the app code, we generated a class signature for ad-call-site code using a similar approach of software bertilonage~\cite{bertillonage}.
We constructed a string by combining the class name of the invoked methods of an ad library, the name of the invoked methods and the parameter types of the invoked methods. 
This constructed string is the class signature for the ad-call-site code.
At the end of this step, we generated class signatures of ad-call-site classes.

\noindent\textbf{Step 3: Compare class signatures.}
In this step, we compared the generated class signatures and identified the app updates where app developers update ad library or ad ad-call-site code.
We followed the following steps to compare the class signatures of ad libraries and ad ad-call-site code
\begin{itemize}
    \item We compared the class signatures in a particular app update ($U_{i}$) with those in a subsequent app update ($U_{i+1}$)
    \item The signatures were updated in the app update ($U_{i+1}$) if the signature of the app update ($U_{i}$) is different than the signature of the app update ($U_{i+1}$)
\end{itemize}
At the end of this step, we identified the updates of the studied apps where app developers update ad library and ad-call-site code.
For each app (A), we also calculate the probability of updating the code (X),for each ad library integration strategy (S) as follows:
\begin{align*}
    P(A,X,S) = \frac{\#\ of\ updates\ with\ integration\ strategy\ S\ of\ an\ app\ A\ where\ ad code\ X\ is\ updated}{Total\ \#\ of\ updates\ with\ integration\ strategy\ S\ of\ an\ app\ A}
\end{align*}
Here, X can be either ``ad-call-site code'' or ``ad library code''.

\textbf{Identify ad-related emergency updates.}
To identify ad-related emergency updates, we need to identify the emergency updates of the studied apps.
In our study, we define an update ($U_{i}$) as emergency update if the difference between the release time of the update $U_{i}$ and the release time of its preceding update $U_{i-1}$ is 0 day. 
At first, for each update $U_{i}$ of the studied apps, we calculated difference between the release time of the update $U_{i}$ and the release time of the update $U_{i-1}$ in days. 
If the difference value is zero day, we considered the update $U_{i}$ as an emergency update.
Then, we checked the emergency update $U_{i}$ in the list of the identified updates where app developers update ad-call site code or update ad libraries.
At the end of this step, we identified all the emergency ad-related updates.


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.65\textwidth]{Images/RQ3/RQ3_Only_Muliple_Strategy.pdf}
    \caption{The probability of updating an ad library integration strategy. The dotted \textcolor{red}{\textbf{red}} line shows the median value of the probability of updating ad-call-site code.} 
    \label{fig:updates_ad_integration_code}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.65\textwidth]{Images/RQ3/RQ3_Ad_Library_Update.pdf}
    \caption{The probability of updating an ad library integration strategy.The dotted \textcolor{red}{\textbf{red}} line shows the median value of the probability of updating an ad library.} 
    \label{fig:update_ad_lib}
\end{figure}

\noindent\emph{Findings:}

\textbf{App developers migrate and rollback to ad libraries -- highlighting the dynamic nature of the ad market.}
We observe that 9\% of ad-displaying apps migrate from one ad library to another ad library.
We find that 54\% of the identified ad libraries involve in these migration cases (e.g., migrate from an ad library and migrate to an ad library).
In these migration cases, maximum number of apps (17\% of the apps that involve in the migration) migrate from Supersonic ad library to IronSource ad library.
There might be numerous factors (e.g., better app revenue, new features) for this migration from SuperSonic to IronSource that we could not identify but one of the possible reasons might be the merger of SuperSonic and IronSource which only supports IronSource ad library.


Moreover, we observe that 10\% of ad-displaying apps rollback to an ad library.
In these rollback cases, maximum number of apps (24\% of the apps that involve in the rollback cases) rollback to MoPub ad library.
The median number of days that app developers take to rollback an ad library is 64 days.
Although we do not know the exact reason for the migration and rollback cases, this result indicates that the ad market is dynamic and every ad network has an opportunity to gain the market.


\textbf{The probability of updating ad-call-site code is 23\% (median) across all integration strategies, with that probability increasing considerably to 37\% (an increase of 60\%) for ad-displaying apps which use a mixed strategy.}
Figure~\ref{fig:updates_ad_integration_code} shows the probability of updating ad-call-site code for every integration strategy.
We observe that the median probability of updating ad-call-site code for ad-displaying apps which use more than one ad library is twice than the median probability of updating ad-call-site code for ad-displaying apps which use single ad library.
Although mixed integration is a well-controlled strategy where app developers leverage both the self mediation and the external mediation, mixed integration requires more maintenance effort than other ad integration strategies.
As shown in the Figure~\ref{fig:updates_ad_integration_code}, the probability of updating ad-call-site code for the mixed strategy and the self-integration strategy are higher than the external mediation strategy.

We recommend that ad library developers should consider the effort required to maintain the ad-call-site code for mixed and self-mediation strategy and offer more features in the external mediation so that they satisfy the need of app developers. 


\begin{table*}[t!]
\centering
\caption{The identified drivers to update ad-related changes in the emergency updates.}
\label{tab:ad_changes_emergency_updates}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{p{3cm}p{2.0cm}p{5.7cm}}
\toprule
\multicolumn{1}{C{3cm}}{\textbf{Driver category}} &
\multicolumn{1}{C{1.7cm}}{\textbf{Integration strategies}} &
\multicolumn{1}{C{5.7cm}}{\textbf{\textbf{Description (\emph{D}) - Example (\emph{E})}}}\\ \midrule
Improving of \newline ads targeting	            &Mixed	   &\textbf{\emph{D:}} App developers modify code to serve ads to the targeted users.\\
 & &\textbf{\emph{E:}} Developers of ``MeetMe: Chat \& Meet New People'' update the logic to serve ads based on the user's country, region and ethnicity.\\
Changing of layouts	    &Mixed	    &\textbf{\emph{D:}} App developers need to update the layout of the apps because of displaying different ads type (e.g., native ads, interstitial ads)\\
& &\textbf{\emph{E:}} Developers of ``Keep Calm GO Keyboard theme'' update app code to introduce a relative layout for displaying native ads from Facebook Audience Network.\\
Adapting with the\newline APIs of an ad library 	&Mixed,\newline Self mediation	         &\textbf{\emph{D:}}App developers need to change ad-call-site code for adapting to the updated APIs of ad libraries.\\
&  &\textbf{\emph{E:}} Developers of ``Music Free'' need to create an anonymous subclass for implementing the \textit{AdListener} class because of the updated version of Google AdMob.\\
\bottomrule     
\end{tabular}
%}
\end{table*}


\textbf{The probability of updating ad libraries is 26.6\% (median) across all integration strategy. We observe that the probability of updating ad-call-site code because of updating ad libraries is higher for ad-displaying apps that use a self mediation strategy.}
Figure~\ref{fig:update_ad_lib} shows the probability of updating ad libraries across all strategies for integrating more than one ad library.
As shown in the Figure~\ref{fig:update_ad_lib}, we observe that the probability of updating ad libraries is higher for ad-displaying apps that use an external mediation strategy than other strategies.

We further study the app updates where app developer updates ad-call site because of updating ad libraries.
For these updates, we observe that the probability value is higher for apps that use self-mediation and mixed strategy than the probability for apps that use the external mediation.

One possible reasons for having a high probability of updating ad-call-site code for updating ad libraries is that app developers need to update the self-mediator which is written by app developers.
%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.65\textwidth]{Paper/Source_Tex/images/RQ4_Ad_maintenance_both_ad_lib_ad_caller_update}
%    \caption{The percentage of the updates of apps for each integration strategy where app developers update ad library and ad integration code.
%    The dotted \textcolor{red}{\textbf{red}} line shows the median of the percentage of updates.} 
%    \label{fig:both_ad_caller_update_ad_lib}
%\end{figure}


\textbf{11.1\% of the emergency updates contain ad-related changes (either update ad-call site code or update an ad library).}
We observe that all these ad-related emergency updates use self-mediation and mixed strategy.
We manually investigated the code changes of these emergency updates to identify the drivers for ad-related changes.
Table~\ref{tab:ad_changes_emergency_updates} shows the identified three drivers for ad related changes.
Among the identified drivers, changing of layouts is important because prior studies shows that majority of the ad complaints are related to user interface (UI)~\cite{gui2017aspects}.
Hence, ad library developers should provide a dynamic way of displaying ads so that app developers do not need to modify the original app's layout.

\begin{Summary}{}{}
The ad market is dynamic as we observe that app developers migrate and rollback to ad libraries in the evolution of the apps. We observe that app developers need to update ad-call-site code and ad library for the maintenance of ad libraries.
We find that probability of updating ad-call-site for the apps that use a mixed strategy is higher than the probability of updating ad-call-site for apps with the mixed and external mediation.

\end{Summary}




==> setup.tex <==
% ------------- Packages Used --------------------------------------------------
% They help us to produce a better looking document ;-)
% ------------------------------------------------------------------------------

% Comment the following line before compiling the final version
%\synctex
\RequirePackage{fix-cm}

\usepackage{caption}
\usepackage{multirow}
\usepackage{balance}
\usepackage{graphicx}
\usepackage{alltt}
\usepackage{relsize}
%\usepackage{xspace}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{paralist}
\usepackage{pbox}
%\usepackage{cleveref}

\newcommand{\tabitem}{~~\llap{\textbullet}~~}

\usepackage{array}
\usepackage{amsmath}
\usepackage{multirow}
%\usepackage{array}
\usepackage{verbatim}
\usepackage[table]{xcolor}
\usepackage{rotating}

%\usepackage{subcaption}
%\usepackage{subfigure}
\usepackage[tight,footnotesize]{subfigure}

%\usepackage{capt-of}
%\usepackage{pifont}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage[latin1]{inputenc}
%\usepackage{times}
%\usepackage{colortbl}
\usepackage{boxedminipage}
\usepackage{float}
\usepackage{cite}
\usepackage{fancyvrb}

\usepackage{balance}

\usepackage{fancybox}%for \hypobox
\usepackage{listings}
\usepackage{array}
\usepackage{afterpage}
\usepackage{pdflscape}
\usepackage{lscape}
\usepackage{rotating}

\usepackage[T1,hyphens]{url}
%\usepackage[colorlinks,urlcolor=blue]{hyperref}


%\hypersetup{
%	colorlinks=true,
%	linkcolor=blue,
%	filecolor=blue,      
%	urlcolor=blue,
%	citecolor=blue,
%}
%\urlstyle{same}

\usepackage{textcomp}
%\usepackage{latexsym}
%\usepackage{amssymb}
%\usepackage{stmaryrd}
%\usepackage{euscript}
%\usepackage{wasysym}
%\usepackage{pifont}
%\usepackage{manfnt}
%\usepackage{undertilde}
%\usepackage{ifsym}
%\usepackage{tipa}
%\usepackage{txfonts}
%\usepackage{skak}
%\usepackage{skull}
%\usepackage{eurosym}
%\usepackage{yfonts}
%\usepackage{mathdots}
%\usepackage{trsym}
%\usepackage{upgreek}
%\usepackage{chemarr}
%\usepackage{accents}
%\usepackage{nicefrac}
%\usepackage{bm}


%\usepackage{pdfsync}

%   ACM Style
%\usepackage{lcsect}
% ------------------------------------------------------------------------------






% ------------ Color Definitions -----------------------------------------------
% Whatever colors we need
% ------------------------------------------------------------------------------
\definecolor{mygray}{rgb}{0.7,0.7,0.7}
% ------------------------------------------------------------------------------






% ---------- Special commands for annotating the paper's text ------------------
\let\mymarginpar\marginparm
\marginparwidth=1cm
\marginparsep=5pt
\newcommand{\todo}[1]{\textcolor{red}{\textbf{[[#1]]}}}
\def\TODO#1{\noindent\colorbox{yellow}{\bf \textcolor{red}{TODO: #1}}}
\newcommand{\hint}[1]{\textcolor{blue}{\textbf{#1}}}
\def\fig#1{Figure~\ref{#1}}
\def\tab#1{Table~\ref{#1}}
\def\eqn#1{Equation~\ref{#1}}
\def\sec#1{Section~\ref{#1}}

\pagenumbering{arabic}
\newcommand{\reviewer}[1]{\textcolor{DeepPink1}{{\it [Reviewer says: #1]}}}
\newcommand{\safwat}[1]{\textcolor{red}{{\it [\textbf{Safwat says: #1}]}}}
\newcommand{\ian}[1]{\textcolor{blue}{{\it [Ian says: #1]}}}
\newcommand{\nic}[1]{\textcolor{WildStrawberry}{{\it [Nico says: #1]}}}
\newcommand{\ahmed}[1]{\textcolor{orange}{{\it [Ahmed says: #1]}}}
\newcommand{\ahsan}[1]{\textcolor{blue}{{\it \textbf{[Ahsan says: #1]}}}}
\newcommand{\cp}[1]{\textcolor{red}{{\it [Cor-Paul says: #1]}}}
\newcommand{\kla}[1]{\textcolor{red}{{\it [Kla says: #1]}}}

\newcommand{\myfoot}[1]{\footnote{\scriptsize #1}}
\newcommand{\myurl}[1]{\myfoot{\url{#1}}}
\newcommand{\Ra}{{$\Rightarrow$}}
\newcommand{\ra}{{$\rightarrow$}}
\newcommand{\La}{{$\Leftarrow$}}
\newcommand{\la}{{$\leftarrow$}}
\newcommand{\lra}{{$\leftrightarrow$}}
\newcommand{\LRa}{{$\Leftrightarrow$}}
%\newcommand{\todo}{\bram{todo}}

\newenvironment{myindentpar}[1]%
{\begin{list}{}%
         {\setlength{\leftmargin}{#1}}%
         \item[]%
}
{\end{list}}

% \AtBeginDocument{%
%    \renewcommand{\figurename}{Figure}%
%    \newcommand{\subfigureautorefname}{\figureautorefname}%for using subfig
% %   \renewcommand{\tablename}{TABLE}%
%    \renewcommand{\tablename}{Table}%
%    \renewcommand{\subsectionautorefname}{Section}%
%    \renewcommand{\sectionautorefname}{Section}%
% }

% Hypothesis box	
% ------------------------------------------------------------------------------	
\newcommand{\hypobox}[1]{\begin{center}%	
	\noindent\thicklines\setlength{\fboxsep}{7pt}%	
	\cornersize{0}\Ovalbox{\begin{minipage}{3.1in}%	
	\vspace{-0.1cm}
	\textit{#1}
	\vspace{-0.1cm}
	\end{minipage}} \end{center}}	
% ------------------------------------------------------------------------------




% ------------------------- SYMBOLS OF SELF NAMES OFTEN USED -------------------
\newcommand{\APACHE}{{\small APACHE}\xspace}
\newcommand{\BUGZILLA}{{\small BUGZILLA}\xspace}
\newcommand{\ECLIPSE}{{\small ECLIPSE}\xspace}
\newcommand{\ASPECTJ}{{\small ASPECTJ}\xspace}
\newcommand{\JDT}{{\small JDT}\xspace}
\newcommand{\GNU}{{\small GNU}\xspace}
\newcommand{\MOZILLA}{{\small MOZILLA}\xspace}
\newcommand{\THUNDERBIRD}{{\small THUNDERBIRD}\xspace}
\newcommand{\JAVA}{{\small Java}\xspace}
\newcommand{\GNOME}{{\small GNOME}\xspace}
\newcommand{\PG}{{\small PostgreSQL}\xspace}
\newcommand{\SIM}{{\small SimScan}\xspace}


\newcommand{\NEGDIFF}{{\emph{Neg}$_{\text{\emph{Diff}}}$}}



% Anything else, e.g., \NAME{MICROSOFT}
\newcommand{\NAME}[1]{{\small #1}\xspace}
% ------------------------------------------------------------------------------




% ----------------------- Computer Science lol ---------------------------------
% Variable, function, and program names
% ------------------------------------------------------------------------------
\newcommand{\smalltt}[1]{\ifmmode{\mbox{\smaller\texttt{#1}}}\else{\smaller\tt #1}\fi}
\newcommand{\code}[1]{\smalltt{#1}}
\newcommand{\var}[1]{\code{#1}}
\newcommand{\func}[1]{\code{#1}}
\newcommand{\proc}[1]{\code{#1}}
\newcommand{\prog}[1]{\code{#1}}
\newcommand{\type}[1]{\code{#1}}
\newcommand{\progpt}[1]{\code{#1}}

\newcommand{\mypar}[1]{\vspace{.1cm}\noindent \textbf{#1}}
\newcommand{\myxpar}[1]{\vspace{.1cm}\noindent \textbf{#1}\newline}
% ------------------------------------------------------------------------------





% ----------- Things to remember -----------------------------------------------
\newenvironment{mynote}%
{ \medskip
  \noindent
  \let\emph=\textbf
  \begin{boxedminipage}{\columnwidth}\em}%
{ \end{boxedminipage}}
% ------------------------------------------------------------------------------






% -------------------- Use bars ------------------------------------------------
% These macros are for advanced presentation of results by shaded bars only!
% © Tom Zimmermann, 2008
% ------------------------------------------------------------------------------
\newdimen\qdx
\newdimen\qda
\newdimen\qdb
\def\rrrr#1#2#3#4{\newdimen\qd\qd=#4 % length of bar for 1.0
\qdx=\qd\multiply\qdx by 5\divide\qdx by 4
\qda=\qd
\qdb=\qd
\multiply\qda by #1\divide\qda by #3\multiply\qdb by #2\divide\qdb by #3\advance\qdb by -\qda
    \leavevmode\hbox to \qdx{\hfil\vbox{%
    \hbox{\vrule\vbox{\hrule\hbox to 1\qd
            {\vrule depth0pt height0.7ex width \qda\color{mygray}%
 \vrule depth0pt height0.7ex width \qdb\hfill}\hrule}\vrule}
    }\hfil}}
\def\rrr#1#2#3{\rrrr{#1}{#2}{#3}{0.8cm}}
% -------------------------------------------------------------------------






% ------------ Graphics Hacks --------------------------------------------------
% Use these settings if Figures tend to get their one separate pages
% ------------------------------------------------------------------------------
% \renewcommand{\topfraction}{0.85}
% \renewcommand{\textfraction}{0.1}
% \renewcommand{\floatpagefraction}{0.75}
% ------------------------------------------------------------------------------





% ------------------ Biblio Hack -----------------------------------------------
% Use these settings if the References take too much space
% ------------------------------------------------------------------------------
\let\oldthebibliography=\thebibliography
  \let\endoldthebibliography=\endthebibliography
  \renewenvironment{thebibliography}[1]{%
%	\vspace{-0.3cm}
    \begin{oldthebibliography}{#1}%
%	\vspace{-0.2cm}
       \setlength{\parskip}{0ex}%
       \setlength{\itemsep}{0ex}%
%	\bibfont
  }%
  {%
    \end{oldthebibliography}%
  }
% ------------------------------------------------------------------------------





% -------------- Floats Redefined ----------------------------------------------
% Use these settings to change the whitespace between floats and text
% ------------------------------------------------------------------------------

% \setlength\dblfloatsep{1pt}
% \setlength\floatsep{1pt}
% \setlength\textfloatsep{5pt}
% \setlength\dbltextfloatsep{5pt}

% \renewcommand\floatpagefraction{.9}
% \renewcommand\topfraction{.9}
% \renewcommand\bottomfraction{.9}
% \renewcommand\textfraction{.1}
% \setcounter{totalnumber}{50}
% \setcounter{topnumber}{50}
% \setcounter{bottomnumber}{50}
% ------------------------------------------------------------------------------



% The custom defined cell types, I needed this to make the headers centered but the remaining of the column is right or left justified.
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{tikz}
\usetikzlibrary{shapes.geometric,calc}

\newcommand\score[2]{
	\pgfmathsetmacro\pgfxa{#1+1}
	\tikzstyle{scorestars}=[star, star points=5, star point ratio=2.25, draw,inner sep=0.15em,anchor=outer point 3]
	\begin{tikzpicture}[baseline]
	\foreach \i in {1,...,#2} {
		\pgfmathparse{(\i<=#1?"yellow":"gray")}
		\edef\starcolor{\pgfmathresult}
		\draw (\i*1em,0) node[name=star\i,scorestars,fill=\starcolor]  {};
	}
	\pgfmathparse{(#1>int(#1)?int(#1+1):0}
	\let\partstar=\pgfmathresult
	\ifnum\partstar>0
	\pgfmathsetmacro\starpart{#1-(int(#1))}
	\path [clip] ($(star\partstar.outer point 3)!(star\partstar.outer point 2)!(star\partstar.outer point 4)$) rectangle 
	($(star\partstar.outer point 2 |- star\partstar.outer point 1)!\starpart!(star\partstar.outer point 1 -| star\partstar.outer point 5)$);
	\fill (\partstar*1em,0) node[scorestars,fill=yellow]  {};
	\fi
	
	,\end{tikzpicture}
}

\newcommand{\smallnum}[1]{$^{\tiny {\textbf #1}}$}

\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand{\specialcellLeft}[2][t]{%
	\begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

\usepackage{threeparttable, tablefootnote}


% needed packaged for consumer apps 
\usepackage[colorlinks,bookmarksopen,bookmarksnumbered,citecolor=red,urlcolor=red]{hyperref}
\usepackage{ragged2e}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{mathtools}
\definecolor{ao}{rgb}{0.0, 0.0, 0.8}
\definecolor{cyan4}{RGB}{0,139,139}
\definecolor{navy}{RGB}{0,0,128}
\usepackage[most]{tcolorbox}

%Beautiful frames/boxes
\newcommand{\tastycolorbox}[1]{\begin{tcolorbox}[enhanced,left=4pt,right=4pt,top=4pt,bottom=4pt,colback=gray!5,colframe=gray!40!black,before skip=6pt,after skip=6pt]#1\end{tcolorbox}}

\newtcbtheorem{Summary}{\bfseries Summary of RQ}{enhanced,
  coltitle=black,
  top=0.1in,
  attach boxed title to top left=
  {xshift=1.5em,yshift=-\tcboxedtitleheight/2},
  boxed title style={size=small,colback=lightgray}
}{summary}

\newtcbtheorem{Summary_data_charac}{Summary}{enhanced,
	coltitle=black,
	top=0.1in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=gray}
}{Summary_data_charac}

\newtcolorbox[auto counter]{summary}[1][]{title={\bfseries Summary},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}
	
\newtcolorbox[auto counter]{summary_RQ1}[1][]{title={\bfseries Summary of RQ1},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}

\newtcolorbox[auto counter]{summary_RQ2}[1][]{title={\bfseries Summary of RQ2},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}
	
\newtcolorbox[auto counter]{summary_RQ3}[1][]{title={\bfseries Summary of RQ3},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}
